Efficient additive Schwarz preconditioning for hypersingular integral equations on locally refined triangulations

For non-preconditioned Galerkin systems, the condition number grows with the number of elements as well as the quotient of the maximal and the minimal mesh-size. Therefore, reliable and effective numerical computations, in particular on adaptively refined meshes, require the development of appropriate preconditioners. We analyze and numerically compare multilevel additive Schwarz preconditioners for hypersingular integral equations, where 2D and 3D as well as closed boundaries and open screens are covered. The focus is on a new local multilevel preconditioner which is optimal in the sense that the condition number of the corresponding preconditioned system is independent of the number of elements, the local mesh-size, and the number of refinement levels.

==> 04_proof_gmld.tex <==
% !TEX root = hypsingAS.tex

%--------------------------------------------------------------------------------
\subsection{Proof of Theorem~\ref{thm:gmld}}\label{section:proof:gmld}
%--------------------------------------------------------------------------------
Clearly, the abstract analytical setting for additive Schwarz
operators from Section~\ref{sec:as} holds true for the operator
\begin{align}
  \PAS^L = \sum_{\ell=0}^L \sum_{z\in\NN_\ell} \prec_z^\ell
\end{align}
associated to the preconditioner defined in Section~\ref{section:main:gmld}.
We stress that the properties of $(\BB^L)^{-1}$ and $\PPAS$ follow in the same
way as for Theorem~\ref{thm:main}. It thus remains to provide a lower and upper
bound for the operator $\PAS^L$.
\begin{proposition}\label{prop:gmld}
 The operator $\PAS^L$ satisfies
\begin{align}\label{eq:prop:GMLD}
  c \, \enorm{v}^2 \leq \edual{\PAS^L v}v 
 \le C(L+1)\,\enorm{v}^2\quad\text{for all } v\in\XX^L.
\end{align}
The constants $c,C>0$ depend only on $\Gamma$ and the initial triangulation
$\TT_0$.
\end{proposition}
In principle, the proof follow the same lines as in
Section~\ref{section:lower bound}--\ref{section:upper bound}. We sketch the most important
modifications only. Details are left to the reader.


\subsection{Proof of lower bound in~\eqref{eq:prop:GMLD}}
In behalf of Lemma~\ref{lem:stabledec} we have to construct a stable
but arbitrary decomposition of all $v\in\XX^L$ into $v_z^\ell \in\XX_z^\ell =
\linhull\{\eta_z^\ell\}$.
Let $v\in\XX^L$. With the Scott-Zhang operator $J_\ell$ from
Section~\ref{sec:sz} we define
\begin{align}
  v^\ell := (J_\ell-J_{\ell-1})v \quad\text{and}\quad v_z^\ell :=
  v^\ell(z)\eta_z^\ell \quad\text{for all } 0\leq\ell\leq L \text{ and }
  z\in\NN_\ell.
\end{align}
We set $J_{-1}:=0$ and note that $J_L v = v$. Property~\eqref{eq:szprop1b}
implies
\begin{align}
  v^\ell(z) = (J_\ell-J_{\ell-1})v(z) = 0 \quad\text{for all } z\in\NN_\ell
  \backslash\widetilde\NN_\ell.
\end{align}
Thus, $v^\ell\in\widetilde\XX^\ell$ and we have the decomposition
\begin{align}
  v = \sum_{\ell=0}^L \sum_{z\in\NN_\ell} v_z^\ell = \sum_{\ell=0}^L
  \sum_{z\in\widetilde\NN_\ell} v_z^\ell,
\end{align}
which, surprisingly, coincides with the decomposition~\eqref{eq:lb1} from
Section~\ref{section:lower bound}. Therefore, the same proof as in
Section~\ref{section:lower bound} applies in this case.



\subsection{Proof of upper bound in~\eqref{eq:prop:GMLD}}
For the proof of the upper bound we define the set
\begin{align}
  \KK_k(z) := \set{ \ell\in \{0,1,\dots,L\}}{z\in\NN_\ell
  \quad\text{and}\quad \level_\ell(z) = k}.
\end{align}
\begin{lemma}\label{lem:KboundGMLD}
  For all $z\in\NN_L$ and $k\in\N_0$ there holds
  \begin{align*}
    \# \KK_k(z) \leq L + 1.
  \end{align*}
\end{lemma}
\begin{proof}
For any node $z\in\NN_L$, there exist at most $L+1$ indices $0\leq \ell\leq L$ such
that $z\in\NN_\ell$. Thus, $\# \KK_k(z) \leq L+1$.
\end{proof}
We proceed as in Section~\ref{section:upper bound} and provide a similar result
as in Lemma~\ref{lem:hypscs}. However, Lemma~\ref{lem:KboundGMLD} plays an
important role in the proof.
To that end, we define the operator $\QQ_m^L : \XX^L \to \widehat \XX^{m+1}$ by
\begin{align*}
  \QQ_m^L := \sum_{\ell=0}^L \sum_{\substack{z\in\NN_\ell\\ \level_\ell(z) = m}}
  \prec_z^\ell,
\end{align*}
and stress that
\begin{align*}
  \PAS^L = \sum_{m=0}^M \QQ_m^L.
\end{align*}
\begin{lemma}\label{lem:hypscsGMLD}
For all $0\leq m\leq M$, $k\leq m+1$
\begin{align}\label{eq:hypscsGMLD}
  0 \le \edual{\QQ^L_m \widehat v^k}{\widehat v^k} 
 \le\c{csugmld} \,(L+1)\,
  2^{-(m+1-k)} \enorm{\widehat v^k}^2
  \quad\text{for all }\widehat v^k\in\widehat\XX^k.
\end{align}
The constant $\setc{csugmld}>0$ depends only on $\Gamma$ and the initial triangulation $\TT_0$.
\end{lemma}
\begin{proof}
The proof follows the same lines as the proof of Lemma~\ref{lem:hypscs}. The
important modifications consist in replacing $\widetilde\NN_\ell$ by $\NN_\ell$,
$\widetilde\KK_m(z)$ by $\KK_m(z)$, and $\widetilde\QQ_m^L$ by $\QQ_m^L$. 
However, in estimate~\eqref{eq:scs5} a bound for the cardinality of the set $\widetilde\KK_m(z)$ enters. 
Clearly, we have to replace this bound by the bound for $\# \KK_m(z)$ from Lemma~\ref{lem:KboundGMLD}. Therefore, the
factor $L+1$ comes into estimate~\eqref{eq:hypscsGMLD}.
\end{proof}
The rest of the proof is a simple postprocessing of Section~\ref{section:upper
bound}, taking care of the additional factor $L+1$.


